PlantMarkerBench: A Multi-Species Benchmark for Evidence-Grounded Plant Marker Reasoning

Cell-type-specific marker genes are fundamental to plant biology, yet existing resources primarily rely on curated databases or high-throughput studies without explicitly modeling the supporting evidence found in scientific literature. We introduce PlantMarkerBench, a multi-species benchmark for evaluating literature-grounded plant marker evidence interpretation from full-text biological papers. PlantMarkerBench is constructed using a modular curation pipeline integrating large-scale literature retrieval, hybrid search, species-aware biological grounding, structured evidence extraction, and targeted human review. The benchmark spans four plant species -- Arabidopsis, maize, rice, and tomato -- and contains 5,550 sentence-level evidence instances annotated for marker-evidence validity, evidence type, and support strength. We define two benchmark tasks: determining whether a candidate sentence provides valid marker evidence for a gene-cell-type pair, and classifying the evidence into expression, localization, function, indirect, or negative categories. We benchmark diverse open-weight and closed-source language models across species and prompting strategies. Although frontier models achieve relatively strong performance on direct expression evidence, performance drops substantially on functional, indirect, and weak-support evidence, with evidence-type confusion emerging as a dominant failure mode. Open-weight models additionally exhibit elevated false-positive rates under ambiguous biological contexts. PlantMarkerBench provides a challenging and reproducible evaluation framework for literature-grounded biological evidence attribution and supports future research on trustworthy scientific information extraction and AI-assisted plant biology.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction state that the paper introduces PlantMarkerBench, a multi-species benchmark for evidence-based plant marker reasoning, and evaluates open and closed LLMs on this benchmark. The claims are supported by the dataset construction, benchmark tasks, model evaluations, and error analyses reported in the paper.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper includes a limitations and responsible-use discussion covering incomplete literature coverage, dependence on available full-text articles, gene-alias ambiguity, limited human validation scope, and the fact that benchmark labels should not be treated as definitive biological truth without expert review.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not introduce theoretical results, theorems, or formal proofs. It is an empirical dataset and benchmark paper.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper and appendix describe dataset construction, benchmark splits, prompts, model settings, metrics, and commands for reproducing the main evaluations. We also release anonymized code, data, Croissant metadata, prediction files, and result aggregation scripts.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide an anonymized dataset and code artifact for review, including benchmark JSONL files, Croissant metadata with RAI fields, evaluation scripts, model-output files, and documentation. The appendix includes commands to reproduce dataset construction, model evaluation, and table generation.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper specifies the balanced pilot splits, evidence labels, prompt modes, evaluated models, deterministic decoding settings, and metrics. Since the primary experiments are zero-shot/few-shot LLM evaluations rather than model training, optimizer and training hyperparameters are not applicable.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: We do not report error bars because the main evaluations are deterministic LLM inference runs with fixed seeds and temperature 0 on fixed benchmark splits. We instead report exact counts, per-class metrics, prompt ablations, cross-species evaluations, and error taxonomy analyses.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The appendix reports compute and runtime details for local open-model evaluation and API-based closed-model evaluation, including the use of Ollama for local models and API calls for closed models. We also provide scripts and expected output directories.

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The work uses publicly available scientific literature and released model APIs/local models for benchmark construction and evaluation. The submission is anonymized for review and does not involve private personal data, clinical data, or human-subject interventions.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper discusses positive impacts for transparent scientific reasoning benchmarks, literature-based biological curation, and reproducible evaluation of LLMs. It also discusses risks including over-reliance on automatically extracted marker evidence, propagation of literature bias, and misuse of benchmark labels as expert-validated biological facts.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The released artifact contains literature-derived benchmark instances and code, not a new high-risk generative model. We include responsible-use documentation, Croissant RAI metadata, provenance fields, and warnings that outputs are intended for benchmarking and curation support rather than direct biological decision-making.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper cites and documents the public resources used, including PMC full-text sources, species annotation resources, embedding models, open LLMs, and closed-model APIs. Licensing and access information are summarized in the appendix and dataset documentation where available.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: PlantMarkerBench is released with documentation, JSONL schemas, Croissant metadata with Responsible AI fields, benchmark splits, label definitions, prompt templates, limitations, and reproducibility instructions. The review artifact is anonymized.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The work does not involve crowdsourcing or human-subject experiments. Human review refers to expert quality control of literature-derived benchmark instances by the authors/research team, not a study involving human participants.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve human subjects, participant recruitment, interventions, or private human data. Therefore IRB approval is not applicable.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerYes{}
    \item[] Justification: LLMs are central to both the dataset construction pipeline and benchmark evaluation. The paper describes their use for evidence grading, structured reasoning-label generation, and model evaluation, and provides prompts, model settings, and decoding details in the appendix.

\end{enumerate}
